Semisimplicity and weight-monodromy for fundamental groups

Let X be a smooth, geometrically connected variety over a p-adic local field. We show that the pro-unipotent fundamental group of X (in both the etale and crystalline settings) satisfies the weight-monodromy conjecture, following Vologodsky. We deduce (in the etale setting) that Frobenii act semisimply on the Lie algebra of the pro-unipotent fundamental group of X, and (in the crystalline setting) that the same is true for a K-linear power of the crystalline Frobenius. We give applications to the representability and geometry of the Selmer varieties appearing in the Chabauty-Kim program, even in cases of bad reduction.

==> modules.tex <==
\section{Mixed $(\varphi, N)$-modules}
In this section, we fix $q\in \mathbb{Z}_{>1}$.

We say that an algebraic integer $\alpha\in \overline{\mathbb{Q}}$ is a $q$-Weil number if there exists $i\in \mathbb{Z}$ such that $|\alpha|_\sigma=q^{i/2}$ for any embedding $\sigma: \overline{\mathbb{Q}}\hookrightarrow \mathbb{C}$; in this case we say that $\alpha$ is a $q$-Weil number of weight $i$.

\begin{defn}
Let $k$ be a field of characteristic zero. A $(\varphi, N)$-module over $k$ is a finite-dimensional $k$-vector space $V$  along with an endomorphism $$N: V\to V$$ and an automorphism $$\varphi:V\to V$$ such that $$N\varphi=q\varphi N,$$ and such that all the generalized eigenvalues of $\varphi$ acting on $V_{\bar k}$ are $q$-Weil numbers.
\end{defn}
Note that $N$ is necessarily nilpotent.

If $V_1, V_2$ are $(\varphi,N)$-modules, we endow $$V_1\otimes_k V_2$$ with a $(\varphi, N)$-module structure with $$N(v_1\otimes v_2)=N(v_1)\otimes v_2+v_1\otimes N(v_2) \text{ and } \varphi(v_1\otimes v_2)=\varphi(v_1)\otimes \varphi(v_2).$$  If $W$ is a $(\varphi,N)$-module, we endow its $k$-dual $W^\vee$ with a $(\varphi,N)$-module structure via $$N(\psi)=-\psi\circ N,\varphi(\psi)=\psi\circ\varphi^{-1}$$ for $\psi\in W^\vee$.    The category of $(\varphi, N)$-modules has an internal Hom, given by $$\underline{\on{Hom}}(V_1, V_2)=V_1^{\vee}\otimes_kV_2.$$

If $V$ is a $(\varphi, N)$-module, let $V^i$ be the maximal $\varphi$-stable subspace of $V$ such that the generalized eigenvalues of $\varphi|_{V^i_{\bar k}}$ are $q$-Weil numbers of weight $i$.  Then by Galois descent, $$V=\bigoplus_{i\in \mathbb{Z}} V^i.$$

Note that if $v\in V$ is a $\varphi$-eigenvector with eigenvalue $\lambda$, then $$\varphi Nv=q^{-1}N\varphi v= q^{-1}\lambda Nv,$$ so $N$ induces a map $$V^i\to V^{i-2}.$$

\begin{defn}
A $(\varphi, N)$-module $V$ is \emph{pure of weight j} if the map $$N^r: V^{j+r}\to V^{j-r}$$ is an isomorphism for all $r\geq 0$.  A $(\varphi, N)$-module $V$ with an increasing $\mathbb{Z}$-indexed filtration $$\cdots \subset F^iV\subset F^{i+1}V\subset \cdots,$$ called the \emph{weight filtration}, is \emph{mixed} if the filtration $F^\bullet$ is exhaustive and separated, preserved by $\varphi, N$, and $\on{gr}^{j}_{F^\bullet} V$ is pure of weight $j$ for all $j$.  The set of \emph{weights} of $V$, denoted $\on{wt}(V)$, is defined as $$\on{wt}(V):=\{j\in \mathbb{Z}\mid \on{gr}^j_{F^\bullet}V\not=0\}.$$
\end{defn}

If $V, W$ are mixed $(\varphi, N)$-modules, $V\otimes W, V^\vee$, and hence $\underline{\on{Hom}}(V, W)$ are mixed $(\varphi, N)$-modules, filtrations given by the usual constructions on filtered vector spaces.  One can check that $$\on{wt}(\underline{\on{Hom}}(V, W))=\{i-j\mid i\in \on{wt}(W), j\in \on{wt}(V)\}.$$ A morphism in the category of mixed $(\varphi, N)$-modules is a linear map commuting with $\varphi, N$, and preserving $F^\bullet$.

The category of mixed $(\varphi, N)$-modules, endowed with these operations, is a symmetric closed compact Abelian category [PROOF].  The unit object $\mathbf{1}$ has underlying vector space $k$, with $N=0, \varphi=\on{id}$ and $$F^i\mathbf{1}=\begin{cases} \mathbf{1} & \text{ if } i\geq 0\\ 0 & \text{ if }  i<0.\end{cases}$$

\begin{theorem}\label{linear-algebra-theorem}
Let $V_1, V_2$ be mixed $(\varphi, N)$-modules, and suppose that for all $i\in \on{wt}(V_1), j\in \on{wt}(V_2)$, we have $i<j$.  Then any extension
$$0\to V_1\to W\to V_2\to 0$$ 
of mixed $(\varphi, N)$-modules splits as a sequence of $k[\varphi]$-modules.
\end{theorem}
\begin{remark}
Note that such sequences do not necessarily split as $k\langle \varphi, N\rangle/(N\varphi-q\varphi N)$-modules.  For example, let $V=k^2$, $$N=\begin{pmatrix} 0 & 1\\  0 & 0\end{pmatrix}, \varphi = \begin{pmatrix} q^{-1} & 0 \\  0 & 1\end{pmatrix}.$$  Let $F^{-2}V=F^{-1}V=\on{Span}\left\{\begin{pmatrix} 1 \\ 0\end{pmatrix}\right\}$, $F^iV=V$ for $i\geq 0$, and $F^iV=\{0\}$ for $i<-2$.  Then the short exact sequence $$0\to F^{-2}V\to V\to V/F^{-2}V\to 0$$ is a non-split exact sequence of mixed $(\varphi, N)$-modules, and $\on{wt}(F^{-2}V)=-2$, whereas $\on{wt}(V/F^{-2}V)=0$.
\end{remark}
\begin{remark}
Suppose $V_1, V_2$ are pure $(\varphi, N)$-modules with $\on{wt}(V_1)>\on{wt}(V_2)$.  Then it is not true that any extension of left $k\langle \varphi, N\rangle/(N\varphi-q\varphi N)$-modules  $$0\to V_1\to W\to V_2\to 0$$ splits as an exact sequence of $k[\varphi]$-modules.  For example, one may take $W=k^3,$ with $$N=\begin{pmatrix} 0 & 1 & 0\\ 0 & 0 & 0 \\ 0 & 0 & 0\end{pmatrix}, \varphi = \begin{pmatrix} 1 & 0 & 1 \\ 0 & q & 0 \\ 0 & 0 & 1\end{pmatrix},$$ and let $V_1=\on{Span}\left\{\begin{pmatrix} 1 \\ 0\\0\end{pmatrix}, \begin{pmatrix} 0 \\ 1 \\ 0\end{pmatrix}\right\}$, $V_2=W/V_1$; $V_1$ is pure of weight $2$, whereas $V_2$ is pure of weight $0$.  In other words, the ordering on weights in Theorem \ref{linear-algebra-theorem} is necessary; it does not suffice that $\on{wt}(V_1)\cap \on{wt}(V_2)=\emptyset$.
\end{remark}
Before proving Theorem \ref{linear-algebra-theorem}, we need a lemma.
\begin{lemma}\label{basic-computation-lemma}
Let $j, r$ be integers with $j<0$ and $r\geq 0$, and let $V$ be the left $k\langle \varphi, N\rangle/(N\varphi-q\varphi N)$-module with $k$-basis $\{f_{q^{j+r}}, f_{q^{j+r-1}}, \cdots f_{q^{j-r}}\}$,  where $$N(f_{q^{i}})=f_{q^{i-1}}, \varphi(f_{q^i})=q^if_{q^i}.$$ Here we set $f_{q^{j-r-1}}=0$ by convention.  Let $\mathbf{1}$ be the left $k\langle \varphi, N\rangle/(N\varphi-q\varphi N)$-module with underlying vector space $k$ and with $\varphi=\on{Id}, N=0$, as above.  Then any extension $$0\to V\to W\to \mathbf{1}\to 0$$ of left  $k\langle \varphi, N\rangle/(N\varphi-q\varphi N)$-modules splits as an extension of $k[\varphi]$-modules.
\end{lemma}
\begin{proof}
If $j+r<0$, $1$ does not appear as a generalized eigenvalue of $\varphi$ acting on $V$, so the result is trivial.  Thus we may assume $j+r\geq 0$.

Suppose $W$ is such an extension.  Let $e\in W$ be any element of $W$ not in $V$.  Then for some $\{a_i\}, \{b_i\}\subset k$, we have $$\varphi(e)=e+\sum a_i f_{q^i} \text{ and } N(e)=\sum b_i f_{q^i}.$$  Thus $$N(\varphi(e))=\sum_j b_j f_{q^j}+\sum_i a_if_{q^{i-1}} \text{ and }q\varphi(N(e))=\sum_i b_iq^{i+1}f_{q^i}.$$  Equating the coefficients of $f_{q^{-1}}$, we see that $a_0+b_{-1}=b_{-1},$ and thus $a_0=0$.  Now set $c_0=0$, and for $i\not=0$, set $$c_i=\frac{a_i}{1-q^i}.$$ Then direct computation shows that 
\begin{align*}
\varphi\left(e+\sum c_i f_{q^i}\right)&=e+\sum a_i f_{q^i}+\sum_{i\not=0} \frac{a_iq^i}{1-q^i}f_{q^i}\\
&=e+\sum_{i\not=0} \frac{a_i}{1-q^i}f_{q^i}\\
&=e+\sum c_i f_{q^i}
\end{align*}
and hence $e+\sum c_i f_{q^i}$ is fixed by $\varphi$ and thus induces a splitting of the exact sequence, as desired.
\end{proof}
\begin{remark}
If we equip $V$ is the statement of Lemma \ref{basic-computation-lemma} with the filtration $F^iV=V$ for $i\geq j, F^iV=0$ for $i<j$, then $V$ is a mixed $(\varphi, N)$-module, with $\on{wt}(V)=\{j\}$.
\end{remark}
\begin{proof}[Proof of Theorem \ref{linear-algebra-theorem}]
Let $$0\to V_1\to W\to V_2\to 0$$ be a short exact sequence as in the statement of the theorem.  Then there is a short exact sequence of mixed $(\varphi, N)$-modules \begin{equation}\label{sequence-to-split} 0\to \underline{\on{Hom}}(V_2, V_1)\to \underline{\on{Hom}}(V_2, W)\to \underline{\on{Hom}}(V_2, V_2)\to 0.\end{equation}
Then fixing an element $e\in \mathbf{1}$, there is a canonical map of mixed $(\varphi, N)$-modules $\mathbf{1}\to \underline{\on{Hom}}(V_2, V_2)$, sending $e$ to $\on{id}_{V_2}$.  We obtain an exact sequence of mixed $(\varphi, N)$-modules \begin{equation} \label{sequence-to-split-2} 0\to \underline{\on{Hom}}(V_2, V_1)\to \widetilde W\to \mathbf{1}\to 0\end{equation} by taking the fiber product of sequence \ref{sequence-to-split} with this map, i.e. the rightmost square in the diagram 
$$\xymatrix{
0\ar[r] & \underline{\on{Hom}}(V_2, V_1)\ar[r] & \underline{\on{Hom}}(V_2, W)\ar[r] & \underline{\on{Hom}}(V_2, V_2)\ar[r] & 0\\
0\ar[r] & \underline{\on{Hom}}(V_2, V_1)\ar[r] \ar@{=}[u]& \widetilde W\ar[r] \ar@{^(->}[u]_s& \mathbf{1}\ar[r] \ar@{^(->}[u]^{e\mapsto \on{id}} & 0
}$$
is Cartesian.  

We first claim that it suffices to split sequence \ref{sequence-to-split-2} as a sequence of $k[\varphi]$ modules.  Indeed, let $$s: \widetilde W\to \underline{\on{Hom}}(V_2, W)$$ be the natural inclusion, and let $\iota: \mathbf{1}\to \widetilde W$ be the required $\varphi$-equivariant splitting.  Then $s\circ \iota(e)\in \underline{\on{Hom}}(V_2, W)$ is a $\varphi$-equivariant splitting of sequence \ref{sequence-to-split}.

Now, we show that sequence \ref{sequence-to-split-2} does indeed split $\varphi$-equivariantly.  By our assumption on the weights of $V_1, V_2$, the weights of $\underline{\on{Hom}}(V_2, V_1)$ are strictly negative.  Thus it suffices to show that if $U$ is a mixed $(\varphi, N)$-module with strictly negative weights, then any extension of mixed $(\varphi, N)$-modules $$0\to U\to T\to \mathbf{1}\to 0$$ splits as a sequence of $k[\varphi]$-modules.  

Without loss of generality, we may assume $k$ is algebraically closed. We proceed by induction on the dimension of $U$.  If $U=0$, the result is trivial.  Otherwise, let $i$ be minimal such that $F^iU$ is nonzero. Let $f\in F^iU$ be a $\varphi$-eigenvector with eigenvalue $\lambda$ a $q$-Weil number of weight $j$, such that $j$ is maximal among all weights appearing as eigenvalues of $\varphi$ acting on $F^iU$. Let $U'=\on{Span}\{f, N(f), N^2(f), \cdots\}\subset U$.  We set $F^{s}U'=0$ for $s<i$ and $F^sU'=U'$ for $s\geq i$, so that $U'$ is a mixed $(\varphi, N)$-module, with $\on{wt}(U')=\{i\}$.  The natural inclusion $U'\to U$ is a morphism of mixed $(\varphi, N)$-modules.

The extension $$0\to U/U'\to T/U'\to \mathbf{1}\to 0$$ splits as an extension of $k[\varphi]$-modules by the induction hypothesis.  Thus it suffices to show that any extension of $(\varphi, N)$-modules $$0\to U'\to T'\to \mathbf{1}\to 0$$ splits $\varphi$-equivariantly.  If $\lambda$ is not a power of $q$, this is trivial, as $1$ is not an eigenvalue of $\varphi: U'\to U'$.  If $\lambda$ is a power of $q$, this is precisely the statement of Lemma \ref{basic-computation-lemma}, completing the proof.
\end{proof}
\begin{lemma}\label{mixed-extensions}
Any extension of mixed $(\varphi, N)$-modules (in the category of filtered $k\langle \varphi, N\rangle/(N\varphi-q\varphi N)$-modules) is mixed.
\end{lemma}
\begin{proof}
This is \cite[Lemma 21]{vologodsky} [OK, I see how to prove this, but Vologodsky omits the proof so we should probably do it].
\end{proof}
